Path Integral Monte Carlo Simulation of Superfluid Ring Lattices

The goal of this work is to lay the groundwork to construct and characterize a quantum device; which we refer to as a superfluid ring lattice; that could serve as a multi-qubit system in the future. Accordingly, a mathematical framework, called the Integer Lattice Method (ILM), is exploited to construct a two-dimensional optical landscape which could facilitate a superfluid ring qubit. The Integer Lattice Method allows one to design and explore both periodic and quasi-periodic structured coherent wave interference patterns. Furthermore, the formalism allows for a direct link to experimental realization. The lattices obtained from ILM can be investigated using WA-PIMC. In particular, the spatial and superfluid density at equilibrium are observables of interest to obtain our objective. In this thesis, the ab-initio Path Integral Monte Carlo Worm algorithm is implemented with the future aim of investigating the construction of superfluid ring lattices. It is written in independent and interchangeable modules in the novel programming language Julia. To ensure scalability, a custom nearest-neighbour algorithm is added. The simulation software is benchmarked by comparing it with exact analytical results from the non-interacting Bose gas model. Emerging issues with our implementation of the Worm algorithm are identified and thoroughly investigated. Finally, some preliminary results on the equilibrium density distribution of the found ILM lattices are presented and discussed.

==> Backmatter/Acknowledgement.tex <==
% \documentclass[../main.tex]{subfiles} % if uncomment than it will build only the subfile. However, I want it to build always the main                          
% \graphicspath{{\subfix{../}}}
% \begin{document}

\chapter*{Acknowledgement}
\addcontentsline{toc}{chapter}{Acknowledgement}%
\todo[inline]{Dmitry}

% \end{document}



==> Chapter_2/Quasicrystal.tex <==
\section{Ultracold atoms in Optical Lattice}
% \subsection{2D Quasicrystal}
% \todo[inline]{\url{https://youtu.be/kdOXLbvg09M}}
% Assume we have grasped all the fundamental models we wish to comprehend. What should we do next? A reductionist would be satisfied. The job is all done. However, one could argue that this is insufficient. New physics can emerge as the system's complexity increases. A simple solution would be to expand the system's size. Nevertheless, this does not always work. The addition of one, ten, or a hundred lattice sites could increase the complexity of a system. However, renormalization group theory \cite{Kenneth1983} suggest that in most cases, the complexity will converge. In many systems, once we've scaled past a certain point, increasing the system will only result in more of the same. As a result, if one seeks a complex system, it has to possess a non-trivial structure at all lengthscales. This is where quasicrystals enter the picture.

% By definition, a 2D quasicrystal is a two-dimensional lattice structure that is ordered, i.e., there exist a spatial symmetry or correlation, but is not periodic, as there exist no one irreducible unit cell where the space can be tiled in. In nature, such an aperiodic tiling was only first found in 1984 by \citet{Shechtman1984} by observing the electron diffraction patterns of an Al-Mn alloy shown in Figure \ref{fig: Quasicrystal}\subref{fig: quasicrystal diffraction pattern}. As can be seen, we have highly well-defined and sharp Bragg Peaks, implying that there is long-range order. However, we also have a five-fold rotational symmetry. This violated the crystallographic restriction theorem, which was an observational statement that a crystal's rotational symmetries are confined to two-fold, three-fold, four-fold, and six-fold. As a result, Shechtman received the Nobel Prize in Chemistry in 2011 for this discovery.
% \begin{figure}[H]
%     \centering
%     \begin{subfigure}[c]{.49\textwidth}
%     \includegraphics[width=\linewidth]{Chapter 2/Figures/Al71Ni24Fe5_TEM.jpg}
%     \phantomsubcaption \label{fig: quasicrystal diffraction pattern}
%     \end{subfigure}
%     \begin{subfigure}[c]{.49\textwidth}
%     \includegraphics[width=\linewidth]{Chapter 2/Figures/Al71Ni24Fe5_TEM.jpg}
%     \phantomsubcaption \label{fig: natural quasicrystal}
%     \end{subfigure}
%     \caption{\subref{fig: quasicrystal diffraction pattern} An icosahedrite ($Al_{86\%}Mn_{14\%}$) electron diffraction pattern generated by directing an electron beam down a fivefold axis of symmetry. Taken from \cite{FigIcosahedrite}. \subref{fig: natural quasicrystal} Taken from \cite{Bindi2015}.}
%     \label{fig: Quasicrystal}
% \end{figure}

==> Preamble/Titlepage/Backcover.tex <==

\thispagestyle{empty}
\sffamily
%
\begin{textblock}{191}(113,-11)
{\color{blueline}\rule{160pt}{5.5pt}}
\end{textblock}
%
\begin{textblock}{191}(168,-11)
{\color{blueline}\rule{5.5pt}{59pt}}
\end{textblock}
%
\begin{textblock}{183}(-24,-11)
\textblockcolour{}
\flushright
\fontsize{7}{7.5}\selectfont
\textbf{Institute for Theoretical Physics}\\
Celestijnenlaan 200D box 2415\\
3000 LEUVEN, BELGI\"{E}\\
tel. +32 16 32 72 32\\
https://fys.kuleuven.be/itf/contact\\
\end{textblock}
%
\begin{textblock}{191}(154,-7)
\textblockcolour{}
\includegraphics*[height=16.5truemm]{Covers/sedes.png}
\end{textblock}
%
\begin{textblock}{191}(-20,235)
{\color{bluetitle}\rule{544pt}{55pt}}
\end{textblock}


==> Preamble/Titlepage/Frontcover.tex <==
\thispagestyle{empty}
\newcommand{\form}[1]{\scalebox{1.087}{\boldmath{#1}}}
\sffamily
%
\begin{textblock}{191}(-24,-11)
\colorbox{green}{\hspace{139mm}\ \parbox[c][18truemm]{52mm}{\textcolor{white}{FACULTY OF SCIENCE}}}
\end{textblock}
%
\begin{textblock}{70}(-18,-19)
\textblockcolour{}
\includegraphics*[height=19.8truemm]{Covers/LogoKULeuven.png}
\end{textblock}
%
\begin{textblock}{160}(-6,63)
\textblockcolour{}
\vspace{-\parskip}
\flushleft
\fontsize{40}{42}\selectfont \textcolor{bluetitle}{Path Integral Monte Carlo of Superfluid Ring Crystals}\\[1.5mm]
\fontsize{20}{22}\selectfont Building Quantum Matter with Optics
\end{textblock}
%
\begin{textblock}{82}(50,103)
\textblockcolour{}
\vspace{-\parskip}
\flushleft
% \fbox{\parbox{79mm}{The background can be left blank or you can insert an image (maximum height 10 cm, width variable, mind author’s rights…). NO logos (you can use the logos inside the manuscript, but not on front or back cover). \textit{Delete this textbox.}}}
\end{textblock}
%
\begin{textblock}{160}(8,153)
\textblockcolour{}
\vspace{-\parskip}
\flushright
\fontsize{14}{16}\selectfont \textbf{Orjan Ameye}
\end{textblock}
%
\begin{textblock}{70}(-6,191)
\textblockcolour{}
\vspace{-\parskip}
\flushleft
Supervisor: \textsl{Prof. Dr. Ir. P. Van Dorpe}\\\vspace{0.3cm}
Co-supervisor: \textsl{Dr. N. Verellen}\\\vspace{0.3cm}
Mentor: \textsl{D. Kouznetsov}
\end{textblock}
%
\begin{textblock}{160}(8,191)
\textblockcolour{}
\vspace{-\parskip}
\flushright
Thesis presented in\\[4.5pt]
fulfillment of the requirements\\[4.5pt]
for the degree of Master of Science\\[4.5pt]
in Physics\\
\end{textblock}
%
\begin{textblock}{160}(8,232)
\textblockcolour{}
\vspace{-\parskip}
\flushright
Academic year 2021-2022
\end{textblock}
%
\begin{textblock}{191}(-24,248)
{\color{blueline}\rule{550pt}{5.5pt}}
\end{textblock}
%
\vfill
\newpage

